Learning to Discover Novel Visual Categories via Deep Transfer Clustering

We consider the problem of discovering novel object categories in an image collection. While these images are unlabelled, we also assume prior knowledge of related but different image classes. We use such prior knowledge to reduce the ambiguity of clustering, and improve the quality of the newly discovered classes. Our contributions are twofold. The first contribution is to extend Deep Embedded Clustering to a transfer learning setting; we also improve the algorithm by introducing a representation bottleneck, temporal ensembling, and consistency. The second contribution is a method to estimate the number of classes in the unlabelled data. This also transfers knowledge from the known classes, using them as probes to diagnose different choices for the number of classes in the unlabelled subset. We thoroughly evaluate our method, substantially outperforming state-of-the-art techniques in a large number of benchmarks, including ImageNet, OmniGlot, CIFAR-100, CIFAR-10, and SVHN.

==> scratch.tex <==
Nonetheless, 
%It will be exciting to enable the machines to automatically learn novel (unseen) image categories without annotations, given some (seen) image categories with annotated instances. 
We aim to tackle this challenge in this paper. In particular, given a labeled dataset $D^l = \{(x^l_1, y^l_1), ..., (x^l_n, y^l_n) \}$ with $n$ images, and an unlabeled dataset $D^u = \{ x^u_1, ..., x^u_m\}$ with $m$ images, where the category space of $D^l$ (e.g., cat, dog) may not be the same with that of $D^u$ (e.g., people, car), our objective is to automatically partition images in $D^u$ into $k$ categories. 








In the first stage, we conduct supervised metric learning with labeled data, resulting in a general feature extractor which can project a data point into a feature space. It is essential to learn a proper non-linear embedding function, $f_{\theta}(x_i)$, to map an image $x_i$ into a discriminative feature space, where features of instances from the same category are close to each other, while features of instances from different categories are far away from each other. We take a convolutional neural network as our embedding function, which we train with a supervised loss (e.g., cross-entropy loss, triplet loss, prototypical loss, etc) on the labeled data. 

In the second stage, we learn categorical prototypes and finetune the feature extractor on unlabeled data with unsupervised loss. To obtain more compact feature representation for clustering, we introduce a linear layer to project the feature produced by the feature extractor into a lower dimention. In particular, we map the feature into another feature space with the dimension equal to the number of categories in the unlabeled data. However, in practice, the number of categories in the unlabeled data may not always be known, we thus propose a simple yet effective way to estimate the number of categories in the feature space.

\begin{figure*}[t] \centering
    \includegraphics[width=0.7\textwidth]{figures/arch.pdf}\\
    \caption{Our model for novel category discovery. It consists of a feature extractor, a linear layer, and a prototype module.} \label{fig:network}
\end{figure*}

\subsection{Clustering assignment}
Assuming the category number (e.g., $k$) of unlabeled data is known a priori, we simultaneously learn $K$ prototypes (i.e., cluster centers) $\left\{\mu_{j}\right\}_{j=1}^{K}$  and finetune the parameters $\theta$ of the embedding function $f_{\theta}$, following deep embedded clustering (DEC)~\cite{Xie16_DEC}. To obtain more compact feature representation, we add an additional linear layer on top of $f_{\theta}$ to project the feature space with a dimension equal to the number of categories. Let the dimension of $f_{\theta}(x)$ be $d$, we have $d\times k$ parameters for the additional linear projection, and $k \times k$ parameters for the prototypes. Similar to~\cite{Maaten09learning}, we adopt the Student's $t$ distribution to measure the similarity between a feature embedding $z_i$ and a prototype $\mu_{j}$. The probability of an instance $i$ belonging to cluster $j$ is defined by 
\begin{equation}
q_{i j}=\frac{(1+\left\|z_{i}-\mu_{j}\right\|^{2} / \alpha)^{-\frac{\alpha+1}{2}}}{\sum_{j^{\prime}}(1+\left\|z_{i}-\mu_{j^{\prime}}\right\|^{2} / \alpha)^{-\frac{\alpha+1}{2}}} , 
% \label{eq:q_ij}
\end{equation}
where $z_{i}=f_{\theta}(x_{i})$ and $\alpha$ are the degrees of freedom of the Student’s $t$-distribution. We set $\alpha$ to $1$ for all experiments.

Following~\cite{Xie16_DEC}, we introduce an auxiliary target distribution $p_i$ given by (\ref{eq:p_ij}) to train our model. The target distribution is constructed by first raising $q_i$ to the second power and then normalizing by the frequency per cluster. Raising $q_i$ to the second power will sharpen the distribution, and thus improve the cluster purity, while the normalization is expected to prevent larger clusters from distorting the hidden feature space.

\begin{equation}
p_{i j}=\frac{q_{i j}^{2} / \sum_{i} q_{i j}}{\sum_{j} q_{i j}^{2} / \sum_{i} q_{i j}} .
\label{eq:p_ij}
\end{equation}

With the soft assignment $q_i$ and target distribution $p_i$, the model can then be learned by minimizing the KL divergence between them. The loss can be written as 

\begin{equation}
L= \sum_{i} \sum_{j} p_{i j} \log \frac{p_{i j}}{q_{i j}} .
\label{eq:kl}
\end{equation}



